On the competition between rotation and variable viscosity in a Darcy-Brinkman model

In the present paper, the onset of thermal convection in a uniformly rotating Darcy-Brinkman porous medium saturated by a variable viscosity fluid is investigated and the competing interplay between rotation and temperature-dependent viscosity is then analysed. %It is well-known in literature that rotation inhibits the onset of vertical motions within the fluid, whereas variable viscosity that depends on temperature may facilitate the onset of instability. In literature it has been proved that considering a variable viscosity fluid saturating a porous medium does not produce any additional oscillating motions at the onset of convection. In this direction, similar results have been obtained in [1], where the authors prove the validity of the principle of exchange of stabilities in a rotating porous medium. Here, it is shown numerically that the combined effect of rotation and variable viscosity may lead to the occurrence of oscillatory convection. This result is remarkable and not known in literature, to the best of our knowledge. The stabilising effect of rotation on the onset of convection is recovered, while it is shown that the effect of variable viscosity on the behaviour of the critical Rayleigh number depends on the choice of the Taylor number. Nonlinear analysis is performed via the energy method and sufficient condition for the stability of the basic solution is determined. Proximity of the results from the linear and nonlinear analyses is obtained thanks to numerical techniques, i.e. Chebyshev-tau method and golden section method.

==> mybib.tex <==
@article{dongarra,
  title={{Chebyshev tau-QZ algorithm methods for calculating spectra of hydrodynamic stability problems}},
  author={Dongarra, J. J. and Straughan, B. and Walker, D. W.},
  journal={Applied Numerical Mathematics},
  volume={22},
  number={4},
  pages={399--434},
  year={1996},
  publisher={Elsevier}}

@article{arnone2023chebyshev,
  title={Chebyshev-$\tau$ method for certain generalized eigenvalue problems occurring in hydrodynamics: a concise survey},
  author={Arnone, G. and Gianfrani, J. A. and Massa, G.},
  journal={The European Physical Journal Plus},
  volume={138},
  number={3},
  pages={281},
  year={2023},
  publisher={Springer}}
@article{bourne2003,
  title={{Hydrodynamic stability, the Chebyshev tau method
and spurious eigenvalues}},
  author={Bourne, D.},
  journal={Continuum Mech. Thermodyn.},
  volume={15},
  pages={571-579},
  year={2003}}

@article{arnonegianfrani,
  title={Stability of penetrative convective currents in local thermal non-equilibrium},
  author={Arnone, G. and Capone, F. and Gianfrani, J. A.},
  journal={Proc. of R. Soc. A},
  volume={480},
  number={2287},
  pages={20230820},
  year={2024},
  publisher={The Royal Society}
}

@book{lanczos1988,
  title={Applied analysis},
  author={Lanczos, C.},
  year={1988},
  publisher={Courier Corporation}
}

@article{acta2022,
  title={{Natural convection in a fluid saturating an anisotropic porous medium in LTNE: effect of depth-dependent viscosity}},
  author={Capone, F. and Gianfrani, J. A.},
  journal={Acta Mechanica},
  year={2022},
  volume={233},
  pages={4535 - 4548},
  url={https://api.semanticscholar.org/CorpusID:252459631}
}
@article{arnone2023onset,
  title={The onset of penetrative convection in an inclined porous layer},
  author={Arnone, G. and Cantini, G. and Capone, F. and Carnevale, M.},
  journal={Int. J. of Heat and Mass Trans.},
  volume={216},
  pages={124532},
  year={2023},
  publisher={Elsevier}
}
@article{mcfadden,
  title={{Elimination of spurious eigenvalues in the Chebyshev-tau spectral methods}},
  author={McFaden, G. B. and Murray, B. T. and Boisvert, R. F.},
  journal={J. Comput Physics},
  volume={91},
  pages={228-239},
  year={1989}
}
@book{gheorghiu2014spectral,
  title={Spectral methods for non-standard eigenvalue problems: fluid and structural mechanics and beyond},
  author={Gheorghiu, C.},
  year={2014},
  publisher={Springer Science \& Business}
}

@book{adams,
  title={Sobolev spaces},
  author={Adams, R. A. and Fournier, J.},
  year={2003},
  publisher={Elsevier}
}
@article{mulone1997,
  title={{The rotating B{\'e}nard problem: new stability results for any Prandtl and Taylor numbers}},
  author={Mulone, G. and Rionero, S.},
  journal={Cont. Mech. and Therm.},
  volume={9},
  number={6},
  pages={347--363},
  year={1997},
  publisher={Springer}
}
@article{RioneroMulone1987,
  title={{On the nonlinear stability of the rotating B\'enard problem via the Lyapunov direct method}},
  author={Mulone, G. and Rionero, S.},
  journal={J. of math. analysis and applications},
  volume={144},
  number={1},
  pages={109--127},
  year={1989},
  publisher={Elsevier},
}

@article{CaponeGentile2000,
  title={On the influence of rotation in convective instabilities in porous media},
  author={Capone, F. and Gentile, M.},
  journal={Ricerche di Matematica},
  volume={49},
  pages={193--211},
  year={2000}
}

@book{straughan2013,
  title={The energy method, stability, and nonlinear convection},
  author={Straughan, B.},
  volume={91},
  year={2013},
  publisher={Springer Science \& Business Media}
}
@book{Galdi1985,
	author = {Galdi, G. P. and Rionero, S.},
	year = {1985},
	title = {{Weighted Energy Methods in Fluid Dynamics and Elasticity}},
	publisher = {Springer},
}
@article{galdi1985exchange,
  title={Exchange of stabilities, symmetry, and nonlinear stability},
  author={Galdi, G. P. and Straughan, B.},
  journal={Archive for rational mechanics and analysis},
  volume={89},
  pages={211--228},
  year={1985},
  publisher={Springer-Verlag}
}

@article{straughan2006global,
  title={Global nonlinear stability in porous convection with a thermal non-equilibrium model},
  author={Straughan, B.},
  journal={Proc. of  R. Soc. A},
  volume={462},
  number={2066},
  pages={409--418},
  year={2006},
  publisher={The Royal Society London}
}
@article{straughan2023nonlinear,
  title={{Nonlinear stability for convection with temperature dependent viscosity in a Navier--Stokes--Voigt fluid}},
  author={Straughan, B.},
  journal={The European Physical Journal Plus},
  volume={138},
  number={5},
  pages={438},
  year={2023},
  publisher={Springer}
}
@article{gianfrani2022,
  title={{Onset of convection in LTNE Darcy--Brinkman anisotropic porous layer: Cattaneo effect in the solid}},
  author={Capone, F. and Gianfrani, J. A.},
  journal={International Journal of Non-Linear Mechanics},
  volume={139},
  pages={103889},
  year={2022},
  publisher={Elsevier}
}
@article{extensiongolden,
  title={{An extension of golden section algorithm for n-variable functions with MATLAB code}},
  author={Rani, G. and Jayan, S. and Nagaraja, K. V. },
  journal={IOP Conference Series: Materials Science and Engineering},
  year={2019},
  volume={577}
}

@article{vadasz1998, title={Coriolis effect on gravity-driven convection in a rotating porous layer heated from below}, 
volume={376}, 
journal={Journal of Fluid Mechanics}, 
author={Vadasz, P.}, 
year={1998}, 
pages={351–375}
}


@ARTICLE{NB,
  author  = {Nield, D.A. and Bejan, A.},
  title   = {Convection in {Porous} {Media}},
  journal = {5th edn. New York, NY: Springer}, 
  volume  = {},
  year    = {2017},
  pages   = {}
}

@misc{website1,
    howpublished = {\url{https://www.engineeringtoolbox.com/ethylene-glycol-d_146.html}}
}

@misc{website2,
    howpublished = {\url{https://wiki.anton-paar.com/it-it/olio-motore/}}
}
@article{torrance,
  title={Thermal convection with large viscosity variations},
  author={Torrance, K. E. and Turcotte, D. L.},
  journal={Journal of Fluid Mechanics},
  volume={47},
  number={1},
  pages={113--125},
  year={1971},
  publisher={Cambridge University Press}
}
@article{joseph,
  title={Variable viscosity effects on the flow and stability of flow in channels and pipes},
  author={Joseph, D. D.},
  journal={The Physics of Fluids},
  volume={7},
  number={11},
  pages={1761--1771},
  year={1964},
  publisher={AIP Publishing}
}
@article{rajagopal2009stability,
  title={{Stability analysis of the Rayleigh--B{\'e}nard convection for a fluid with temperature and pressure dependent viscosity}},
  author={Rajagopal, K. R. and Saccomandi, G. and Vergori, L.},
  journal={Zeitschrift f{\"u}r angewandte Mathematik und Physik},
  volume={60},
  pages={739--755},
  year={2009},
  publisher={Springer}
}


@article{straughan2004,
  title={Global stability for convection when the viscosity has a maximum},
  author={Diaz, J. and Straughan, B.},
  journal={Linear and Nonlinear Stability in non-standard Theories of Fluid Dynamics},
  volume={16},
  pages={347--352},
  year={2004}
}
@article{hughes,
  title = {{Rapidly rotating Maxwell-Cattaneo convection}},
  author = {Hughes, D. W. and Proctor, M. R. E. and Eltayeb, I. A.},
  journal = {Phys. Rev. Fluids},
  volume = {7},
  issue = {9},
  pages = {093502},
  year = {2022},
  publisher = {American Physical Society}
}
@article{vadasz2021centrifugal,
  title={Centrifugal buoyancy in a rotating fluid layer next to and distant from the rotation axis},
  author={Vadasz, P.},
  journal={Physics of Fluids},
  volume={33},
  number={3},
  year={2021},
  publisher={AIP Publishing}
}
@article{taylor1923,
  title={Stability of a Viscous Liquid Contained between Two Rotating Cylinders},
  author={Taylor, G. I.},
  journal={Philosophical Transactions of the Royal Society A},
  year={1923},
  volume={223},
  pages={289-343}
}
@book{chandra,
  author  = {Chandrasekhar, S.},
  title   = {Hydrodynamic and hydromagnetic stability},
  publisher = {Dover Publicationas}, 
  volume  = {},
  year    = {1981},
  pages   = {}
}


@book{drazin,
  author  = {Drazin, P. G. and Reid, W. H.},
  title   = {Hydrodynamic stability},
  publisher = {Cambridge University Press}, 
  volume  = {},
  year    = {2004},
  pages   = {}
}
@article{gianfrani2020,
  title={{Optimal stability thresholds in rotating fully anisotropic porous medium with LTNE}},
  author={Capone, F. and Gentile, M. and Gianfrani, J. A.},
  journal={Transport in Porous Media},
  volume={139},
  pages={185--201},
  year={2021},
  publisher={Springer}
}
@article{straughan2023rotating,
  title={{Rotating convection in a higher gradient Navier--Stokes fluid}},
  author={Straughan, B.},
  journal={The European Physical Journal Plus},
  volume={138},
  number={7},
  pages={1--13},
  year={2023},
  publisher={Springer}
}
@book{vafai,
  title={Handbook of porous media},
  author={Vafai, K.},
  year={2005},
  publisher={Crc Press}
}
@article{capone2022thermal,
  title={{Thermal convection for a Darcy-Brinkman rotating anisotropic porous layer in local thermal non-equilibrium}},
  author={Capone, F. and Gianfrani, J. A.},
  journal={Ricerche di Matematica},
  volume={71},
  number={1},
  pages={227--243},
  year={2022},
  publisher={Springer}
}
@article{vadasz2019instability,
  title={{Instability and convection in rotating porous media: A review}},
  author={Vadasz, P.},
  journal={Fluids},
  volume={4},
  number={3},
  pages={147},
  year={2019},
  publisher={MDPI}
}
@ARTICLE{Capone2020,
       author = {{Capone}, F. and {De Luca}, R. and {Gentile}, M.},
        title = {Coriolis effect on thermal convection in a rotating bidispersive porous layer},
      journal = {Proc. R. Soc. A},
         year = {2020},
       volume = {476},
       number = {2235},
        pages = {20190875}
}

@article{straughan1986,
  title={Stability criteria for convection with large viscosity variations},
  author={Straughan, B.},
  journal={Acta Mechanica},
  year={1986},
  volume={61},
  pages={59-72}
}
@article{kassoy1975,
  title={Variable viscosity effects on the onset of convection in porous media},
  author={Kassoy, D. R. and Zebib, A.},
  journal={The Physics of Fluids},
  volume={18},
  number={12},
  pages={1649--1651},
  year={1975},
  publisher={AIP Publishing}
}
@article{capone2022natural,
  title={{Natural convection in a fluid saturating an anisotropic porous medium in LTNE: effect of depth-dependent viscosity}},
  author={Capone, F. and Gianfrani, J. A.},
  journal={Acta Mechanica},
  volume={233},
  number={11},
  pages={4535--4548},
  year={2022},
  publisher={Springer}
}

@ARTICLE{barletta,
       author = {{Barletta}, A. and {Mulone}, G.},
        title = "{{The energy method analysis of the Darcy-B{\'e}nard problem with viscous dissipation}}",
      journal = {Continuum Mechanics and Thermodynamics},
         year = {2021},
       volume = {33},
       number = {1},
        pages = {25-33}
}

@article{park2013stably,
  title={{The stably stratified Taylor--Couette flow is always unstable except for solid-body rotation}},
  author={Park, J. and Billant, P.},
  journal={Journal of Fluid Mechanics},
  volume={725},
  pages={262--280},
  year={2013},
  publisher={Cambridge University Press}
}
@article{park2017instabilities,
  title={{Instabilities and transient growth of the stratified Taylor--Couette flow in a Rayleigh-unstable regime}},
  author={Park, J. and Billant, P. and Baik, J.},
  journal={Journal of Fluid Mechanics},
  volume={822},
  pages={80--108},
  year={2017},
  publisher={Cambridge University Press}
}
@article{Gianfrani2023,
  title={{Effect of Vadasz term on the onset of convection in a Darcy–Brinkman anisotropic rotating porous medium in LTNE}},
  author={Capone, F. and Gianfrani, J. A.},
  journal={Continuum Mechanics and Thermodynamics},
  year={2022},
  volume={35},
  pages={1911 - 1926}
}
